Lightweight Embedded FPGA Deployment of Learned Image Compression with Knowledge Distillation and Hybrid Quantization

Learnable Image Compression (LIC) has shown the potential to outperform standardized video codecs in RD efficiency, prompting the research for hardware-friendly implementations. Most existing LIC hardware implementations prioritize latency to RD-efficiency and through an extensive exploration of the hardware design space. We present a novel design paradigm where the burden of tuning the design for a specific hardware platform is shifted towards model dimensioning and without compromising on RD-efficiency. First, we design a framework for distilling a leaner student LIC model from a reference teacher: by tuning a single model hyperparameters, we can meet the constraints of different hardware platforms without a complex hardware design exploration. Second, we propose a hardware-friendly implementation of the Generalized Divisive Normalization - GDN activation that preserves RD efficiency even post parameter quantization. Third, we design a pipelined FPGA configuration which takes full advantage of available FPGA resources by leveraging parallel processing and optimizing resource allocation. Our experiments with a state of the art LIC model show that we outperform all existing FPGA implementations while performing very close to the original model.

==> leftovers.tex <==
**** Experiments section ****


\begin{figure}[htbp]
  \centering
  \includegraphics[width=1\columnwidth]{figures/patch.PNG}   
  \caption{Proposed Hardware Patch Processing }
  \label{fig:patch_process}
\end{figure}


Table.\ref{tab:FPS_numbers_patch_vs_modular} provides system level FPS numbers on a model mapped to the FPGA where Patch FPS provides the FPS performance  per patch for each module, modular FPS provides the overall FPS for each module for an 720p input, as is the case for all performance metric evaluations, the main decoder computational load is higher and as such consistently has lower FPS.

\begin{table}[htb]
\centering
\caption{Modular Codec Performance per Full 720p Input Using 256x256 Patch Blocks}
\renewcommand{\arraystretch}{1.2} % Increase row height for better readability
\begin{tabular}{ccc} % Use 'c' for centered columns
\hline
\textbf{Model} & \textbf{Patch FPS} & \textbf{Modular FPS} \\
\hline
\textit{Main Encoder} & 78.85 & 26.99 \\
\textit{Main Decoder} & 54.12 & 16.38 \\
\textit{Hyper Encoder} & 243.12 & 80.67 \\
\textit{Hyper Decoder} & 242.60 & 79.46 \\
\textit{Entropy Model} & 1144.0 & 376.2 \\
\hline
\end{tabular}
\label{tab:FPS_numbers_patch_vs_modular}
\end{table}






\begin{figure}[htbp]
  \centering
  \includegraphics[width=1\columnwidth]{figures/BD_MP.png} 
  \caption{BD rates and PSNR for Mixed Precision models}
  \label{fig:BD_MP}
\end{figure}

Fig.\ref{fig:BD_MP} shows the Bjontegaard-delta (BD) rate and PSNR results for the proposed knowledge distillation scheme, where the teacher model is used as reference. A 0.08 drop in PSNR can be observed in the K160 model accompanied with a 6.5\% BD-rate increase, these losses are traded off for a 15 FPS increase. We will explore the advantage of the proposed KD scheme further in the ablation study where we do not use the KD scheme and merely reduce the model size. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.8\columnwidth]{figures/change_design.png}  % Adjust width as needed
  \caption{The design choice trade-offs which allow us to achieve realtime operations and 70 FPS using the knowledge distillation scheme on Lambda=0.0075
}
  \label{fig:change_design}
\end{figure}
